Numerical Verification of Affine Systems with up to a Billion Dimensions

Affine systems reachability is the basis of many verification methods. With further computation, methods exist to reason about richer models with inputs, nonlinear differential equations, and hybrid dynamics. As such, the scalability of affine systems verification is a prerequisite to scalable analysis for more complex systems. In this paper, we improve the scalability of affine systems verification, in terms of the number of dimensions (variables) in the system. The reachable states of affine systems can be written in terms of the matrix exponential, and safety checking can be performed at specific time steps with linear programming. Unfortunately, for large systems with many state variables, this direct approach requires an intractable amount of memory while using an intractable amount of computation time. We overcome these challenges by combining several methods that leverage common problem structure. Memory is reduced by exploiting initial states that are not full-dimensional and safety properties (outputs) over a few linear projections of the state variables. Computation time is saved by using numerical simulations to compute only projections of the matrix exponential relevant for the verification problem. Since large systems often have sparse dynamics, we use Krylov-subspace simulation approaches based on the Arnoldi or Lanczos iterations. Our method produces accurate counter-examples when properties are violated and, in the extreme case with sufficient problem structure, can analyze a system with one billion real-valued state variables.

==> basic_efficiency.tex <==

\subsection{Method Efficiency}
\label{ssec:basic_efficiency}
Although the computation time at each step is reduced, we must still compute (and store) the matrix
exponential at the first step, which for very large systems may be still be impractical.
%
We can overcome this by using the numerical simulation method of computing the matrix exponential as 
described in Section~\ref{ssec:basic_efficiency}.
%
This method computes the matrix exponential one column at a time using simulations.
%
Rather using this to construct the full matrix exponential, we can instead project the simulation at each step
onto the key directions, and then only store the projected values.

For example, consider a million-dimensional verification problem with a thousand discrete time steps 
and one key direction ($n = 1000000$, $s = 1000$, $k = 1$). 
%
A single numerical simulation will produce a sequence of $n$-dimensional state vectors
$\mathbf{x}_0, \mathbf{x}_1, \ldots, \mathbf{x}_s$, one at a time.
%
Each state vector is $n \times 1$, requiring 8 MB of storage (assuming double-precision floating point).
%
At each step in the simulation $j$, 
we compute and store $\mathbf{k} \mathbf{x}_j$, which is a single scalar.
%
After completing all $n$ simulations for all $s$ steps, the total amount of memory for storing the result is 
just the size of the basis matrix multiplied by the number of steps, which
is 8 GB.
%
In contrast, storing the $n \times n$ matrix exponential at the first step would need 8 TB of memory, more than
what is available on most current systems.




%%%%%%%%%%%%%%%%%%%%%%%%

The dimension of the initial states $i$, can often be significantly smaller than the number of system variables.
%
We can combine these fixed variables together so that, if only $i$ dimensions are initially 
variable (not fixed), we only need to do $i + 1$ simulations.
%
%This can be viewed as a second projection, from the space of initial state uncertainty 
%onto the full state space of our system.

In order to combine fixed variables, we exploit the principle of superposition of solutions of linear 
systems~\cite{duggirala2016parsimonious,girard2006efficient}.
%
Superposition means that solutions can be added together as initial states are added together.
%
For example, if a linear system starting at initial state $(1, 0, 0, \ldots, 0)^T$
reaches a state $\mathbf{x}'$ after $t$ time, and the same linear system starting at initial state
$(0, 1, 0, \ldots, 0)^T$ reaches a different state $\mathbf{x}''$ after $t$ time, then the system 
starting at the summed initial state $(1, 1, 0, \ldots, 0)^T$, after $t$ time, will reach the 
state $\mathbf{x}' + \mathbf{x}''$.

This additivity property can also help with computing sums of projected states.
%
In the timed harmonic oscillator of Section~\ref{ssec:ha}, three of the variables are initially fixed values
($x_0 = -5$, $t_0 = 0$, $a_0 = 1$).
%
In the previous method, we would compute a simulation for each of these variables from the corresponding unit vector
in the identity matrix, projecting onto the key direction $\mathbf{k}$ at each step.
%
In the LP constraints, these projected values would be multiplied by the fixed initial state values (for example, in
Figure~\ref{sfig:projecting_key}, initial state constraints set $x_0$ to $-5$).
%
In a sense, this is also taking advantage of superposition, where the solution from 
$(x_0, y_0, t_0, a_0)^T = (1, 0, 0, 0)^T$ is used to compute the solution from $(-5, 0, 0, 0)^T$.
%
The new approach exploits additivity by running a single simulation 
from the combined initial state of fixed terms $(x_0, 0, t_0, a_0)^T$, and computing 
its projection onto $\mathbf{k}$ at each step.
%
In the LP, we remove the $x$, $t$, and $a$ variables and their associated constraints, and add
a new fixed-term-effect variable $f$ which is set to $1$.
%
In $f$'s column in the basis matrix, we place the projected value of the simulation from the combined initial state.
%
The set of linear constraints after this transformation is shown in Figure~\ref{sfig:combining_fixed}.

In the extreme case, where every variable is initially fixed, then all of the columns of the basis matrix can
be combined into the fixed term, which is computed from a single simulation.
%
This essentially means that, if you trust the numerical accuracy of your simulation engine, 
verification of a system with no uncertainty amounts to performing a single discrete-time simulation and then 
checking the unsafe condition at each step.

There is a connection between combining fixed variables and 
reachability with affine representations of low-dimensional polytopes~\cite{han2006reachability}.
%
In this method, a low-dimensional initial polytope is projected to high-dimensional space at each
step in the computation.
%
Similarly, in our approach, if only a small number of dimensions $i$ are initially 
variable (not fixed), this can be viewed as an initial polytope with $i$ dimensions, which we project into the higher
$n$-dimensional space using $i$ columns of the matrix exponential, and then project again down onto the key directions.
%
The double-projection process is encoded as a single step within the basis matrix.






There are many different ways to compute the matrix exponential~\cite{moler2003nineteen}.
%
Generally, the methods implemented in off-the-shelf libraries use a series expansion.
%
To save time, since $e^{A2t} = e^{At} ~ e^{At}$, we can compute the matrix exponential once for the first
time step, and then use matrix-matrix multiplication to obtain its value at subsequent steps.
%
Although this may be less accurate than doing the series expansion at every step, 
for the systems we have considered and for thousands of discrete steps, its accuracy has been
sufficient (better than the tolerances used in the numeric LP solver).

An alternative method to compute the matrix exponential uses numerical simulations (method $5$~\cite{moler2003nineteen}).
%
The matrix exponential is computed one column at time by using the fact that 
$e^{At} = e^{At} ~ \mathbf{I}_{n \times n} = e^{At} ~ (\mathbf{e}_1 | \mathbf{e}_2 | \ldots | \mathbf{e}_n)$. 
%
The $j$th column of $e^{At}$ is equal to $e^{At} \mathbf{e}_j$, where $\mathbf{e}_j$ is 
the $j$th column of the identity matrix.
%
The value of $e^{At} \mathbf{e}_j$, however,  is just the solution of the linear system $\dot{x} = Ax$ at time $t$ from 
initial state $x(0) = \mathbf{e}_j$.
%
To compute this, we perform a numerical simulation with an off-the-shelf method such as
Runge-Kutta.
%
For example, for the matrix exponential shown in the basis matrix of Figure~\ref{sfig:full_constraints}, the first 
column $(-0.707, -0.707, 0, 0)^T$ could be computed by using a simulation of the
system from initial state $\mathbf{e}_1=(1, 0, 0, 0)^T$ up to time $\frac{3\pi}{4}$.

This process is repeated for each column of the identity matrix to compute the full matrix exponential.
%
When many discrete time steps are required, and when $A$ is a large sparse matrix, this approach can be 
faster than a series-based method, even with the matrix-matrix multiplication speedup.
%
This method has been used to verify safety of systems with thousands of dimensions using 
a few hours of computation time~\cite{bak2017arch}.
%
The simulation approach to computing the matrix exponential will serve as the basis for some of the 
methods developed later in this paper, since it provides a way to decompose the large matrix exponential 
computation into a series of smaller computations for each column.


==> heat_nonsym.tex <==
\subsection{Nonsymmetric 3D Heat Diffusion}
\label{ssec:heat_nonsym}

We analyzed a non-symmetric version of the 3D Heat Diffusion system, where the initially heated region is replaced by 
a permanent heater is present along on the bottom of the block $z = 0.0$, along the 2D rectangle where $x \in [0.0, 0.4]$ 
and $y \in [0.0, 0.2]$.
%
We analyze the system up to time 500, with a time step of 0.5 ($s=1000$).
%
The plot of the temperature reachable at the center for the 10x10x10 version (1000 dimensions) and the 
100x100x100 version (1 million dimensions) is shown in Figure~\ref{fig:heat_reach}.
%
Table~\ref{tab:heat} shows the maximum temperature reached at the center of the block as
we vary the number of mesh points per axis $m$.

The scalability bottleneck for this system comes from the memory needed for the Arnoldi algorithm as given in
Equation~\ref{eq:memory_arnoldi}.
%
The 200x200x200 version exhausted memory before completing.


\begin{figure}[tb]
%\begin{floatrow}
%\ffigbox{%
    \includegraphics[width=0.48\textwidth]{figures/heat_reach.png}
%}{%
  \caption{The spatial discretization affects the temperature reachable at the center.}%
  \label{fig:heat_reach}%
  \end{figure}

%\capbtabbox{%
\begin{table}
  \caption{3D Heat Diffusion with $n=m^3$ Dimensions}
    \label{tab:heat}
\begin{tabular}{@{}llll@{}}
\toprule
\bf{$m$} ~~~ & Temp ~~~ & $k$ ~~~ & \bf{Runtime} \\
\midrule
\input{figures/heat_summary.dat}
\bottomrule
\end{tabular}

\end{table}
%
%\end{floatrow}



==> heli_single.tex <==
\subsection{Replicated Helicopter with Combined Error Condition}
\label{ssec:heli_single}

We considered a modified version of the helicopter benchmark, where the unsafe condition is changed to check the 
average of the $x^j_8$ variables, making the output dimension $o=1$. 
%
From Equation~\ref{eq:memory_basis}, we now would exhaust main memory storing the basis matrices 
when $h \approx 7.15$ million, a system with about 200 million dimensions. 

Analysis of the runtime for this version of the benchmark is shown in Figure~\ref{fig:heli_singlekey}.
%
In the larger systems, solving the LP becomes the bottleneck, making improvements
to the Arnoldi portion less important.

\begin{figure}[t]
  \centering
%\begin{floatrow}
%\ffigbox{%
    \includegraphics[trim={0 0 0 0em}, clip, width=0.7\textwidth]{figures/heli_singlekey.pdf}
%}{%
    \caption{With smaller output space $o=1$, the \texttt{Krylov} method verify the replicated helicopter
system with about 300 thousand dimensions in 10 minutes (top of the y axis).}
    \label{fig:heli_singlekey}
\end{figure}


\begin{table}[b]
  \centering
  \caption{Replicated Helicopter Runtime (sec) with $o=1$}
  \label{tab:heli_singlekey}
\begin{tabular}{@{}llll@{}}
\toprule
{\bf Dims} & {\bf Expm} & {\bf Mult} & {\bf Kry} \\
\midrule
\input{figures/singlekey_summary.dat}
\bottomrule
\end{tabular}

\end{table}
%
%\end{floatrow}

